Modelling Child Learning and Parsing of Long-range Syntactic Dependencies

This work develops a probabilistic child language acquisition model to learn a range of linguistic phenonmena, most notably long-range syntactic dependencies of the sort found in object wh-questions, among other constructions. The model is trained on a corpus of real child-directed speech, where each utterance is paired with a logical form as a meaning representation. It then learns both word meanings and language-specific syntax simultaneously. After training, the model can deduce the correct parse tree and word meanings for a given utterance-meaning pair, and can infer the meaning if given only the utterance. The successful modelling of long-range dependencies is theoretically important because it exploits aspects of the model that are, in general, trans-context-free.

==> scrap.tex <==
for wh- and polar questions, it occurs around point 500, and for negated wh- and polar questions, it occurs near the end of training. The analysis in the earlier Figure \ref{fig:example-parse-tree} depicts an instance of this, of how already acquired lexical and syntactic knowledge can facilitate rapid acquisition of a new lexical item. 
%TODO: say standard thing for 'why does negwh jump up towards the end'? A: by then it's alreayd learnt a lot of syntax, see Figure 8

There, the word ``music'' has never been observed before, and so the corresponding nodes of the tree have very low probability. However, by that stage, the learner is confident in the analysis of the rest of the sentence, so it still gives high probability to the depicted analysis. This high probability means that the co-occurrence counts for $music$ and ``music'' get a large update, leading to a large increase in the CPP.

We observe that, prior to this point at which it begins making the fully correct analysis of a certain construction, the learner is still often able to infer the correct meaning for the utterance using a non-standard parse tree.
%, leveraging spurious ambiguity. 
For example, if a verb and argument have been observed together several times, it may interpret the whole verb phrase as a single lexical item (an example of this is in Figure \ref{fig:prog-test-parses}). This could give the correct meaning for the verb phrase, and hence the utterance, but, if such an analysis were made by the learner, it would not facilitate one-trial learning of a novel verb, because there would be no leaf node that contains just the novel verb word. For example, given the utterance ``he is gorping'', it could analyze ``is gorping'' as a single lexical item, at the expense of the analysis in which ``gorping'' is a leaf. So, although it might acquire the meaning for this entire VP in one trial, it would not do the same for the word ``gorping'' itself. This difference helps explain why we see a smooth trajectory for deducing utterance meaning, (Figure \ref{fig:test-lfs}) but sudden jumps in Figure \ref{fig:one-trial-learning}. 

The fact that this jump occurs late for negated questions (both polar and wh-), means that it takes longer for the learner to start making fully correct analyses for these constructions, in particular, for the sequence of elements auxiliary, negation, subject, verb, which appears in both negated question types. This is consistent with a comparison to Figure \ref{fig:parse-acc-by-type}, which shows that, by training example 3500, the model has already learnt much of the correct syntax cross a variety of constructions.

For progressives, the model never fully reaches the stage of consistently making the correct analysis, and instead keeps most of its probability mass on an analysis in which the copula and verb together form a lexical item, e.g. there is a leaf node with meaning $\lambda x.\lambda y.pres_{3s}(jump_{prog}\; x\; y)$ and word span ``is running''. Some probability mass does fall on the correct analysis in which this node is split into two leaves, one meaning $\lambda p.\lambda z.pres_{3s}(p\; z)$ with word span ``is'', and one with meaning $\lambda x.\lambda.jump_{prog}\; x\; y$ and word span ``running'', and this allows it to partially learn the novel word. The trajectory for progressives in Figure \ref{fig:one-trial-learning} appears to have plateaued. However, due to the rapid nature of our model`s acquisition of this ability, it is possible that, given more data, it would eventually, suddenly, become able for one-trial learning from progressives as from other constructions. 
